Multi-Class Multiple Instance Learning for Predicting Precursors to Aviation Safety Events

In recent years, there has been a rapid growth in the application of machine learning techniques that leverage aviation data collected from commercial airline operations to improve safety. Anomaly detection and predictive maintenance have been the main targets for machine learning applications. However, this paper focuses on the identification of precursors, which is a relatively newer application. Precursors are events correlated with adverse events that happen prior to the adverse event itself. Therefore, precursor mining provides many benefits including understanding the reasons behind a safety incident and the ability to identify signatures, which can be tracked throughout a flight to alert the operators of the potential for an adverse event in the future. This work proposes using the multiple-instance learning (MIL) framework, a weakly supervised learning task, combined with carefully designed binary classifier leveraging a Multi-Head Convolutional Neural Network-Recurrent Neural Network (MHCNN-RNN) architecture. Multi-class classifiers are then created and compared, enabling the prediction of different adverse events for any given flight by combining binary classifiers, and by modifying the MHCNN-RNN to handle multiple outputs. Results obtained showed that the multiple binary classifiers perform better and are able to accurately forecast high speed and high path angle events during the approach phase. Multiple binary classifiers are also capable of determining the aircraft's parameters that are correlated to these events. The identified parameters can be considered precursors to the events and may be studied/tracked further to prevent these events in the future.

==> Introduction.tex <==
\section{Introduction}
The aviation industry brings tremendous amount of social and economic benefits. It has been observed the size of the air transportation industry has doubled every 15 years \cite{aviationbenefit2019}, and was expected to continue growing \cite{market_outlook} prior to COVID-19. In 2018 alone, airlines around the world carried a total of 4.3 billion passengers while the total global economic impact of the industry reached USD 2.7 Trillion in 2016 \cite{aviationbenefit2019}. Furthermore, even though the industry continues to grow and more people are flying everyday, aviation safety has improved over the past decades as seen on Figure~\ref{fig:fatalities}. 

\begin{figure}[h!]
 \centering % Always center your figures and tables.
 \includegraphics[width=0.7\linewidth]{Images/year_in_safety_for_commercial.jpg}
 \caption{Commercial Aviation Fatalities from FY96 to FY19 \cite{FAA_safety}}
 \label{fig:fatalities}
\end{figure}

The number of fatalities for commercial air carriers decreased from 81 per 100 million persons on board in 1996 to 0.6 in 2019, which is below the target rate set by the Federal Aviation Administration (FAA). This reduction is the result of the efforts undertaken by agencies such as the  National Aeronautics and Space Administration (NASA), the Federal Aviation Administration (FAA), the National Transportation Safety Board (NTSB), and others. In particular, these efforts led to better certification standards, better operating procedures, and decision-support systems \cite{model_env_safety}. However, it is important to keep reducing the accident rate even further so that we do not observe a rise in the number of accidents given the industry's expected continued growth \cite{reduce_accident_rate_faa, market_outlook}. In order to significantly improve safety, the aviation industry has been moving towards a proactive approach to safety assessment and vulnerability identification, which consists of characterizing potential risks in terms of anomalies or deviations from nominal operations and the precursors to adverse events. This knowledge can be leveraged to increase awareness of emerging vulnerabilities amongst the operators and be incorporated into automated monitoring tools to flag the risks before they result in a near-miss, incident or accident \cite{aviation_safety_blog}. 

Extensive data collection and advancement in data-mining methodologies are key enablers to proactive risk management in aviation \cite{Logan2008, aviation_safety_blog}. Airline programs such as the Flight Operations Quality Assurance (FOQA) have enabled the creation of large, and heterogeneous data sets. FOQA is a voluntary safety program that is designed to make commercial aviation safer. Data is collected using devices such as Quick Access Recorder (QAR) or directly from Flight Data Recorder (FDR) \cite{FAA_FOQA}. Traditional techniques of flight data analysis have focused on a continuous cycle of data collection from on-board recorders, retrospective analysis of flight-data records, identification of operational safety exceedances, design and implementation of corrective measures, and monitoring to assess their effectiveness. Airlines work with the FAA to reduce and eliminate safety risks, and flight safety divisions within airlines generally use FOQA data to perform exceedence and statistical analyses. Exceedence analysis consist of setting specific limits to the recorded airborne data so that particular parameters that fall outside of the normal operating conditions can be flagged \cite{FAA_FOQA}. The level of exceedence can be programmed for different severities of events. These profiles are used to create distributions of various criteria, which enables airlines to evaluate flight risk levels and trend known vulnerabilities over time \cite{FAA_FOQA}. A validation step at the end of each analysis is performed to determine the nature of corrective actions required and to store valid events in databases for analyzing trends \cite{FAA_FOQA}. 

Research efforts have been made towards advancing the development of data-driven methodologies, applying data science techniques, and using modern machine learning, including deep learning algorithms, in the context of aviation safety \cite{anomaly_detection_review_survey, precursor_jamey, precursor_vijay, precursor_vijay2, survey_data_mining, Matthews2013, Puranik2018_AD, Puranik2019_AD}.
Majority of the data mining effort in aviation is directed at detecting anomalies in aviation data~\cite{MKL, flight_anomaly_dbscan_GT, anomaly_detection_gaussian, flight_anomaly_detection_real_time, Puranik2018_AD, survey_data_mining, vae, corrado} and leveraging unsupervised learning techniques due to lack of labeled data. Data mining has also been applied towards predictive maintenance in aviation~\cite{anomaly_detection_review_survey} and predicting future trajectory states~\cite{puranik2020_towards}. While identifying anomalies is important, it is also critical to investigate the causal factors or precursors to these anomalies or other safety events in order to understand them better and  prevent them in the future. Recent literature has focused on identifying precursors to safety events and anomalies using FOQA data~\cite{precursor_vijay, precursor_jamey, data_driven_precursor}. Precursors can be defined as any event that are correlated to a safety incident and occurs prior the incident itself \cite{precursor_vijay}. They are useful for forecasting safety events, and provide insights to why the event happened. Knowing the precursors can then be used to initiate actions to avoid events from occurring \cite{data_driven_precursor}. Therefore, being able to identify and monitor precursors is an important step towards proactive safety enhancement in aviation operations. One of the main challenges in identification of precursors observed in literature is the lack of subject-matter-expert validated labels for the identified anomalies and safety events. To account for the lack of labels usually encountered, this paper proposes the application of a weakly-supervised learning technique called multi-class multiple-instance learning (MIL)~\cite{li2018multiclass} to detect different multiple adverse events and their precursors.

Considering the above observations, the main aim of this paper is the development of a methodology that leverages highly dimensional aviation data to predict multiple adverse events and discover their precursors. This work will use a flight-level label called a bag-label in MIL terminology to predict the anomalies at the flight-level and identify their precursors along with their occurrence in-time during a flight. The current framework uses a deep learning model constructed as multi-headed convolutional neural network (CNN) where each flight sensor gets its own CNN and the multi-headed architecture is designed to work with the MIL framework. Successful implementation of the methodology uses the flight's data to 1) predict adverse events, and 2) determine the precursors to the predicted adverse events. One major benefit from this framework over current approaches will be the extension of binary classifiers to perform multi-class predictions and the ability to retrieve the precursors with little to no post-processing. Additional benefits will include transferability of the model due its multi-head architecture, knowledge discovery to help analysts find root causes of safety events faster, and relative simplicity of the model to provide better transparency and explainability (compared to previous architectures).
